Exploring Mixed Integer Programming Reformulations for Virtual Machine Placement with Disk Anti-Colocation Constraints

One of the important problems for datacenter resource management is to place virtual machines (VMs) to physical machines (PMs) such that certain cost, profit or performance objective is optimized, subject to various constraints. In this paper, we consider an interesting and difficult VM placement problem with disk anti-colocation constraints: a VM's virtual disks should be spread out across the physical disks of its assigned PM. For solutions, we use the mixed integer programming (MIP) formulations and algorithms. However, a challenge is the potentially long computation time of the MIP algorithms. In this paper, we explore how reformulation of the problem can help to reduce the computation time. We develop two reformulations, by redefining the variables, for our VM placement problem and evaluate the computation time of all three formulations. We show that they have vastly different computation time. All three formulations can be useful, but for different problem instances. They all should be kept in the toolbox for tackling the problem. Out of the three, formulation COMB is especially flexible and versatile, and it can solve large problem instances.

==> heuristics.tex <==
\subsection{Comparison with Heuristics}
\label{sec:heuralgo}

%We compare it with online randomized heuristic algorithms.

We next illustrate concretely some of the advantages of the MIP approach, which were summarized in Section \ref{sec:introduction} earlier. The focus here is to provide evidence that the MIP approach can achieve substantially lower costs than obvious heuristic algorithms. Thus, it is worthwhile to explore the MIP approach and look for different MIP formulations to speed up the computation. Throughout the discussion, we will also point out other advantages of MIP.


Since we are not aware of prior studies on exactly our problem (due to the disk anti-colocation requirements), we developed our own heuristic algorithm. To make our heuristic algorithm an honest benchmark for comparison, we make it aggressive in the sense that it sacrifices computation speed in an attempt to achieve a lower cost. By doing so, its achievable cost can serve as a lower bound for a class of other possible heuristic algorithms that put speed at a higher priority. We also remark that, in this paper, we do not claim contributions on designing an all-around good heuristics for our problem.

%In other words, our heuristic algorithm is likely to be competitive among (future) heuristic algorithms in terms of achieving low cost, because it sacrifices computation time for lower cost.

%We will mostly focus on the advantage with respect to the achievable cost.

%We next make some comments on the advantage of the MIP approach with respect to the achievable cost. The objective is to provide some evidence that the MIP-based approach can achieve substantially lower costs than many heuristic algorithms. Since we are not aware of prior studies on exactly our problem (due to the disk anti-colocation requirements), we had to develop our own heuristic algorithm. To make our heuristic algorithm a useful benchmark for comparison, we make it aggressive in the sense that it sacrifices speed for higher performance. By doing so, its performance can serve as a lower bound for a class of other possible heuristic algorithms that put speed at a higher priority.


%For this paper, we do not claim contributions on designing a good heuristics for our problem. Many heuristics can be easily thought out. But, a heuristic algorithm that works well under one set of parameters may not work well under another set. In general, it is not easy to design a simple heuristic good enough for most cases that can be encountered in practice. Neither is it easy to claim that a heuristic works well for most practical cases, since doing so requires either a theoretical proof or thorough exploration of a large parameter space.

%Our heuristic algorithm is not designed to be fast. Although faster than the MIP algorithms, the heuristic algorithm is not sufficiently scalable for large problems due to the use of exhaustive search. Because of the complexity of our problem, it is not obvious how to design another heuristic algorithm that is both fast and achieves low costs.


\subsubsection{Randomized Heuristic Algorithm}


\begin{algorithm}
\caption{Randomized Heuristic Algorithm}
\label{alg:heur}
\begin{algorithmic}[1]
\STATE permute the {\tt VM\_list}
\FOR{each VM in {\tt VM\_list}}
\STATE scan {\tt used\_PM\_list} to find a PM that can accommodate the VM \label{ln:scan1}
\IF{such a PM is found}
\STATE assign the VM to the PM
\ELSE
\STATE scan {\tt unused\_PM\_list} to find a PM that can accommodate the VM \label{ln:scan2}
\IF{such a PM is found}
\STATE assign the VM to the PM; move the PM to {\tt used\_PM\_list}
\ELSE
\STATE exit \hspace{0.2in} \# the problem is infeasible
\ENDIF
\ENDIF
\ENDFOR
\end{algorithmic}
\end{algorithm}


Our heuristic algorithm is motivated by the general ideas of online randomized algorithms \cite{Tang_ascalable, AAS14, Li20131222} but should achieve much lower costs than the latter due to the use of exhaustive search. In other words, our heuristic algorithm is given more time to search for good solutions than typical online randomized algorithms that immediately place a requested VM to some random PM. The algorithm is summarized in Algorithm \ref{alg:heur}.

The algorithm first randomly permutes the list of all the requested VMs; this emulates the random arrival order of the VM requests. For each VM in the permuted list, an attempt is made to assign the VM to a PM. The PMs are organized into two lists -- the list of {\em used} PMs, which are those PMs already with some assigned VMs, and the list of {\em unused} PMs.

To place a VM, the list of used PMs is searched exhaustively first. If no PM in the used list can accommodate the VM, then the list of unused PMs is checked. Note that, in our model, a PM incurs a constant operation cost regardless of how many VMs are assigned to it. The algorithm's greedy behavior of first checking the used PMs matches the assumption of constant operation costs.\footnote{The discussion also suggests that, if the cost model is different, the current heuristic algorithm may not work well. For instance, if the operation costs of the PMs depend on the load placed on the PMs in some complicated way, then trying to pack VMs to used PMs first may not be the right approach.} Before scanning a PM list, the PM list is randomly permuted to emulate random selection if multiple PMs are suitable for the current VM. Then, the PM list is scanned, and the first PM in the list that can accommodate the VM is selected. This aspect is known as the the first-fit heuristic, which is an often used heuristic \cite{Tang_ascalable, AAS14, Li20131222}.\footnote{We can consider several other alternatives. There is a popular heuristic algorithm known as first-fit-decrease. The VMs are sorted in a decreasing order of the resource requirements. For each VM in the list, the PM list is searched. A VM is placed in the first PM that can accommodate it. Such an algorithm makes sense if the objective is to be able to place all the VMs. On the other hand, if the number of PMs is abundant and the objective is to minimize some cost, then the sorting of the VMs is not necessarily helpful. The results depend on the order in which the PM list is scanned. Another heuristic idea is to sort each PM list in an increasing order of the operation costs and scan the PMs according to that order instead of a random order. This way, cheaper PMs are used with a higher priority. Whether such sorting is beneficial depends on the details of the problem instance, i.e., all the parameters, such as the costs, the resources of the PMs and the requested resources of the VMs.}

%The points are that (i) there is a large number of possible heuristics, and (ii) the performance of a heuristic algorithm sometimes depends critically on the precise values of the problem's parameters, which change from instance to instance. Finding a good heuristic algorithm that works for most problem instances encountered in practice can be difficult or time consuming. On the other hand, the MIP algorithm can be trusted to always yield optimal solutions for all instances that it can solve.

%In scanning either PM list, the order of scanning is uniformly random to emulate random selection. The first PM in the list that can accommodate the VM is selected.

%Our heuristic algorithm is motivated by the general ideas of online randomized algorithms \cite{Tang_ascalable, AAS14, Li20131222} but should achieve much lower costs than the latter due to the use of exhaustive search. In other words, our heuristic algorithm is given more time to search for good solutions than typical online randomized algorithms that immediately place a requested VM to some random PM. Here are some of the details of our heuristic algorithm. Imagine that VM requests arrive dynamically. An online randomized algorithm will assign a requested VM to some random PM one at a time in the arrival order of the VM requests. Note that, in our experiments, all the VMs to be placed are given together in a batch. Our greedy randomized algorithm first randomly permutes the list of all the requested VMs; this emulates the random arrival order of the VM requests. For each VM in the permuted list, an attempt is made to assign the VM to a PM. The greedy aspect is that, for assignment, the list of {\em used} PMs, which are those already with some assigned VMs, is checked first; if the VM cannot be assigned to any PM in the used list, then the list of unused PMs is checked. Note that a PM incurs a constant operation cost regardless of how many VMs are assigned to it. The greedy aspect of the algorithm fits the cost minimization objective. In scanning either PM list, the order of scanning is uniformly random to emulate random selection. The first PM in the list that can accommodate the VM is selected. This aspect is known as the the first-fit heuristic, which is an often used heuristic \revisit{reference}.
%\footnote{There is a popular heuristic algorithm known as first-fit-decrease. The VMs are sorted in a decreasing order of the resource requirements. For each VM in the list, the PM list is searched. A VM is placed in the first PM that can accommodate it. This algorithm makes sense if the objective is to be able to place all the VMs. On the other hand, if the number of PMs is abundant and the objective is to minimize some cost, then the sorting of the VMs is not necessarily helpful. The results depend on the order at which the PM list is scanned. Another heuristic idea is to sort each PM list in an increasing order of the operation costs and scan the PMs according to that order instead of a random order. This way, cheaper PMs are used with a higher priority. Whether such sorting is beneficial depends on the details of the problem instance, i.e., all the parameters, such as the costs, the resource configurations of the PMs and the requested configurations of the VMs. The points are that (i) there is a large number of possible heuristics, and (ii) the performance of a heuristic algorithm sometimes depends critically on the precise values of the problem's parameters, which change from instance to instance. Finding a good heuristic algorithm that works for most problem instances encountered in practice can be difficult or time consuming.}



For each scanned PM (in line \ref{ln:scan1} and \ref{ln:scan2}), our heuristic algorithm checks whether it is possible to assign the currently considered VM to that PM. For vCPU or memory, it is enough to check whether the remaining number of vCPUs or the remaining memory is sufficient for the VM. For disk assignment, the algorithm exhaustively enumerates different disk assignment possibilities and uses the first one that is feasible. As discussed earlier, the disk anti-colocation constraints are the difficult ones to satisfy. Our heuristic algorithm is aggressive in finding a feasible disk assignment. Other practical heuristic algorithms are unlikely to conduct an exhaustive search, since the number of possible disk assignments can sometimes be very large, e.g., millions or more. With exhaustive search, our algorithm will achieve a lower total operation cost.

%For instance, a type-l6 PM has $24$ physical disks and a VM of type i2.8xlarge needs $8$ virtual disks. The number of disk assignment possibilities is $\frac{24!}{(24-8)!}=29,654,190,720$.

Table \ref{tab:summary_I_II} summarizes the costs achieved by the heuristic algorithm, and compares them with the optimal costs. Details are given in the following.


%If the disk assignment (for the currently considered VM and PM) cannot be done after the search, it is because the assignment is infeasible.


%\footnote{For a large datacenter, a scalable online algorithms cannot afford to search through all the used PMs or unused PMs for each VM request. A typical strategy is to randomly sample a few used PMs and, if that does not work out, pick a unused PM with sufficient resources randomly. Our heuristic algorithm should do better in the achievable objective value. A more sophisticated algorithm is to keep track of an ordered list of all the PMs according to certain criterion and assign the VM to the first one on the list that fits. In this case, exhaustive search is needed and scalability is limited. Our heuristic algorithm does not maintain an ordered list because there is no obvious criterion for the order due to the difficult disk exclusivity requirement.}


%\footnote{Checking the feasibility of disk assignment can be done by some standard assignment algorithm, which may be faster than enumeration but still takes some time. Either way, our heuristic algorithm has limited scalability, since in the worst case, there is one disk assignment problem for every PM for every VM request. But, it should achieve a lower cost than more scalable online randomized algorithms that do not check all the PMs for all possible disk assignment possibilities.}



%For brevity, we omit the details.

%The heuristic algorithm is only used to show how much better the optimization approach is in terms of the total cost achieved.

%We develop a randomized heuristic algorithm for solving formulation F1, which can be used as a target of cost comparison with the integer programming approach. The heuristic algorithm is motivated by the general ideas of online randomized algorithms but should achieve much lower costs than the latter due to the use of exhaustive search. In other words, our heuristic algorithm is given more time to search for good solutions than typical online randomized algorithms that immediately place a requested VM to some random PM. The heuristic algorithm is only used to show how much better the optimization approach is in terms of the total cost achieved. Although faster than the integer programming algorithms, the heuristic algorithm is not sufficiently scalable for large problems due to the use of exhaustive search. Because of the complexity of our problem, it is not obvious how to design another heuristic algorithm that both gives high-quality solutions and is fast. For brevity, we omit the details.

\subsubsection{Experiment I -- $70$ VMs and $50$ PMs}

Since our heuristic algorithm involves randomization, we collected the results of $50$ runs (on the same problem instance). The average cost of the $50$ runs is $9913$, more than twice the optimal cost achieved by the MIP algorithm ($4540$). The minimum, maximum and standard deviation of the costs are $6980$, $12000$, and $1074$, respectively. As we argued, when compared with other possible heuristics, our heuristic algorithm is designed to do quite well in terms of the achievable cost. The gaps from the optimal cost are expected to be wider for other heuristic algorithms that do not use exhaustive search. In this problem instance, our heuristic algorithm can solve the problem quickly. The $50$ runs took several seconds all together.

\subsubsection{Experiment II -- $77$ VMs and $70$ PMs}

We ran the heuristic algorithm $50$ times on this problem instance. The resulting average cost is $65105$ and the standard deviation is $3683$. The minimum and maximum costs are $58400$ and $76200$, respectively. On average, the heuristic algorithm results in $44\%$ higher cost than the optimal cost, which is $45300$. Percentage-wise, the heuristic algorithm is doing better here than for the previous problem instance. Part of the reason is that, even in the optimal solution, $38$ out of the $70$ PMs are used and there is not a lot of room for cost saving, in terms of percentage of improvement. Nevertheless, the cost saving {\em in value} by the optimal solution is still much more than that for the previous instance.

\subsubsection{Experiment III -- $1000$ VMs and $1000$ PMs} For this problem instance, the heuristic algorithm produces a mean cost of $150573$, which is much larger than the optimal cost $66040$.

